Iterative Monte Carlo analysis of spin-dependent parton distributions

We present a comprehensive new global QCD analysis of polarized inclusive deep-inelastic scattering, including the latest high-precision data on longitudinal and transverse polarization asymmetries from Jefferson Lab and elsewhere. The analysis is performed using a new iterative Monte Carlo fitting technique which generates stable fits to polarized parton distribution functions (PDFs) with statistically rigorous uncertainties. Inclusion of the Jefferson Lab data leads to a reduction in the PDF errors for the valence and sea quarks, as well as in the gluon polarization uncertainty at $x \gtrsim 0.1$. The study also provides the first determination of the flavor-separated twist-3 PDFs and the $d_2$ moment of the nucleon within a global PDF analysis.

==> tab-sampling.tex <==
\begin{center}
\begin{tabular}{@{\extracolsep{\fill}} ccccccc}
\hline\hline
$f(x,Q^2_0)$ & $n$                      & $a$      & $b$      & $c$      & $d$\\\hline
$\Delta u^+$ & -                        & $[-1,0]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\
$\Delta d^+$ & -                        & $[-1,0]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\
$\Delta s^+$ & $\Delta\Sigma^{(1)}=0.5$ & $[-1,0]$ & $[2,10]$ & $[-1,1]$ & $[-1,1]$\\
$\Delta g$   & $\Delta g^{(1)}=0.5$     & $[-1,0]$ & $[2,10]$ & $[-1,1]$ & $[-1,1]$\\
$D_u$        & 0                        & $[-1,1]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\
$D_d$        & 0                        & $[-1,1]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\
$H_p$        & 0                        & $[-1,1]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\
$H_n$        & 0                        & $[-1,1]$ & $[2,5]$  & $[-1,1]$ & $[-1,1]$\\\hline
\end{tabular}
\end{center}


